BRENDA: Browser Extension for Fake News Detection

Misinformation such as fake news has drawn a lot of attention in recent years. It has serious consequences on society, politics and economy. This has lead to a rise of manually fact-checking websites such as Snopes and Politifact. However, the scale of misinformation limits their ability for verification. In this demonstration, we propose BRENDA a browser extension which can be used to automate the entire process of credibility assessments of false claims. Behind the scenes BRENDA uses a tested deep neural network architecture to automatically identify fact check worthy claims and classifies as well as presents the result along with evidence to the user. Since BRENDA is a browser extension, it facilities fast automated fact checking for the end user without having to leave the Webpage.

==> conclusion.tex <==
\section{Conclusions and Future Work}
In this paper we presented an hierarchical attention mechanism to jointly learn various latent aspect embeddings for news. For example, these latent aspects can be subject, author and domain related to the claim and news articles. This allows us to capture salient vocabulary and complex structure at the document level. Compared to the only claim-text based attention, the attention weights, which are jointly learned guided by both claim text and different latent aspects are more effective for detecting if the claims are True or False. This is apparent from our experiments conducted on Snopes, Politifact and Fever dataset. We also propose an algorithm to extract evidence snippets supporting or refuting the claim from news articles using attention weights at both the word and sentence level from all three models. We show a t-SNE visualization that the learned embeddings are also good predictors of fake news.  We also show examples where the evidence extracted using our latent aspect embeddings are superior to simple word level attention used in \declare. In future, we plan to conduct a detailed user study on the informativeness and interpretability of these evidence snippets.


==> setup.tex <==
\section{Experimental Setup}
We implement SADHAN using TensoFlow framework. We use 10 fold cross validation to evaluate the our model’s performance. We use per-class accuracy, macro F1 score and AUC as performance metrics for evaluation. We used pretrained GloVe embeddings of $100$ dimentions, trained on $6$ billion words. We tuned the parameters using validation set, as a result we use softmax cross entropy with logits as cost function, learning rate of $0.001$ and size of hidden states and cell states of Bi-LSTM units are kept as $200$. for drop out regularization we used  $keep prob = 0.3$.  


